In-Kernel Control-Flow Integrity on Commodity OSes using ARM Pointer Authentication

This paper presents an in-kernel, hardware-based control-flow integrity (CFI) protection, called PAL, that utilizes ARM's Pointer Authentication (PA). It provides three important benefits over commercial, state-of-the-art PA-based CFIs like iOS's: 1) enhancing CFI precision via automated refinement techniques, 2) addressing hindsight problems of PA for in kernel uses such as preemptive hijacking and brute-forcing attacks, and 3) assuring the algorithmic or implementation correctness via post validation. PAL achieves these goals in an OS-agnostic manner, so could be applied to commodity OSes like Linux and FreeBSD. The precision of the CFI protection can be adjusted for better performance or improved for better security with minimal engineering efforts if a user opts in to. Our evaluation shows that PAL incurs negligible performance overhead: e.g., <1% overhead for Apache benchmark and 3~5% overhead for Linux perf benchmark on the latest Mac mini (M1). Our post-validation approach helps us ensure the security invariant required for the safe uses of PA inside the kernel, which also reveals new attack vectors on the iOS kernel. PAL as well as the CFI-protected kernels will be open sourced.

==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}

- Hong.
- Note on GT.
- Brandon Azad at Google Project Zero.

==> cases.tex <==
\section{Case Study: New Attack Vectors}
\label{s:cases}

\PP{Apple iOS.}

XPAC gadget

%ref. pac:mosec19.pdf

\framebox{P1}

\framebox{P2}

\framebox{P3}

\framebox{P4}

%\begin{figure}
%	\include{code/xpac-gadget.c}
%	\coderule
%	\caption{A \cc{xpac}-gadget in iOS 13 that allows an attacker
%		to hijack the control flow of the kernel
%		to an arbitrary function.}
%	\label{fig:xpacGadget}
%\end{figure}

%\figurename{\ref{fig:xpacGadget}}

\PP{PARTS.}



==> code/analyzer.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{//     typesig       objtype, allowed target, refinement}
\PY{k+kt}{void}\PY{p}{(}\PY{o}{*}\PY{p}{)}\PY{p}{(}\PY{k}{struct} \PY{n}{kref} \PY{o}{*}\PY{p}{)}\PY{p}{,} \PY{n}{NONE}\PY{p}{,}       \PY{l+m+mi}{1075}\PY{p}{,}     \PY{n}{retbind}
\PY{n}{irq\PYZus{}handler\PYZus{}t}\PY{p}{,}          \PY{n}{irqaction}\PY{p}{,}  \PY{l+m+mi}{275}\PY{p}{,}      \PY{n}{objbind}
\end{Verbatim}


==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/global-init.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{typedef} \PY{k+kt}{void}\PY{o}{*} \PY{n}{pac\PYZus{}t}\PY{p}{;}
\PY{k}{typedef} \PY{k}{struct} \PY{p}{\PYZob{}}
  \PY{n}{pac\PYZus{}t} \PY{o}{*}\PY{n}{addr}\PY{p}{;}
  \PY{n}{u64} \PY{n}{buildtime\PYZus{}ctx}\PY{p}{;}
  \PY{n}{u64} \PY{n}{runtime\PYZus{}ctx}\PY{p}{;}
\PY{p}{\PYZcb{}} \PY{n}{pac\PYZus{}entry\PYZus{}t}\PY{p}{;}

\PY{k}{extern} \PY{n}{pac\PYZus{}entry\PYZus{}t} \PY{n}{\PYZus{}\PYZus{}pac\PYZus{}start}\PY{p}{[}\PY{p}{]}\PY{p}{;}
\PY{k}{extern} \PY{n}{pac\PYZus{}entry\PYZus{}t} \PY{n}{\PYZus{}\PYZus{}pac\PYZus{}end}\PY{p}{[}\PY{p}{]}\PY{p}{;}

\PY{p}{.}\PY{p}{.}\PY{p}{.}

\PY{k+kt}{void} \PY{n}{\PYZus{}\PYZus{}init} \PY{n}{early\PYZus{}pauth\PYZus{}init}\PY{p}{(}\PY{k+kt}{void}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{n}{pac\PYZus{}entry\PYZus{}t} \PY{o}{*}\PY{n}{ppac}\PY{p}{;}
  \PY{k}{for} \PY{p}{(}\PY{n}{ppac} \PY{o}{=} \PY{n}{\PYZus{}\PYZus{}pac\PYZus{}start}\PY{p}{;} \PY{n}{ppac} \PY{o}{\PYZlt{}} \PY{n}{\PYZus{}\PYZus{}pac\PYZus{}end}\PY{p}{;} \PY{n}{ppac}\PY{o}{+}\PY{o}{+}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n}{pac\PYZus{}t} \PY{n}{addr} \PY{o}{=} \PY{o}{*}\PY{n}{ppac}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{addr}\PY{p}{;}
    \PY{n}{\PYZus{}\PYZus{}asm\PYZus{}\PYZus{}} \PY{n+nf}{\PYZus{}\PYZus{}volatile\PYZus{}\PYZus{}}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{PACIB \PYZpc{}0, \PYZpc{}1}\PY{l+s+se}{\PYZbs{}n}\PY{l+s}{\PYZdq{}}
       \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{=\PYZam{}r}\PY{l+s}{\PYZdq{}}\PY{p}{(}\PY{n}{addr}\PY{p}{)}
       \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s}{r}\PY{l+s}{\PYZdq{}}\PY{p}{(}\PY{n}{ppac}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{buildtime\PYZus{}ctx} \PY{o}{\PYZca{}} \PY{n}{ppac}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{runtime\PYZus{}ctx}\PY{p}{)}\PY{p}{,}
         \PY{l+s}{\PYZdq{}}\PY{l+s}{0}\PY{l+s}{\PYZdq{}}\PY{p}{(}\PY{n}{addr}\PY{p}{)}\PY{p}{)}\PY{p}{;}
    \PY{o}{*}\PY{n}{ppac}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{addr} \PY{o}{=} \PY{n}{addr}\PY{p}{;}
  \PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/keyswitching.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{p}{.}\PY{n}{macro} \PY{n}{kernel\PYZus{}entry}\PY{p}{,} \PY{n}{el}\PY{p}{,} \PY{n}{regsize} \PY{o}{=} \PY{l+m+mi}{64}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
  \PY{n}{mrs\PYZus{}s} \PY{n}{x0}\PY{p}{,} \PY{n}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}
  \PY{n}{mvn} \PY{n}{x0}\PY{p}{,} \PY{n}{x0}
  \PY{n}{msr\PYZus{}s} \PY{n}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}\PY{p}{,} \PY{n}{x0}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}

\PY{n}{macro} \PY{n}{kernel\PYZus{}exit}\PY{p}{,} \PY{n}{el}\PY{p}{,} \PY{n}{regsize} \PY{o}{=} \PY{l+m+mi}{64}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
  \PY{n}{mrs\PYZus{}s} \PY{n}{x20}\PY{p}{,} \PY{n}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}
  \PY{n}{mvn} \PY{n}{x20}\PY{p}{,} \PY{n}{x20}
  \PY{n}{msr\PYZus{}s} \PY{n}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}\PY{p}{,} \PY{n}{x20}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\end{Verbatim}


==> code/keyswitching.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n+na}{.macro} \PY{n+no}{kernel\PYZus{}entry}\PY{p}{,} \PY{n+no}{el}
  \PY{n+nf}{mrs\PYZus{}s} \PY{n+no}{x0}\PY{p}{,} \PY{n+no}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}
  \PY{n+nf}{mvn} \PY{n+no}{x0}\PY{p}{,} \PY{n+no}{x0}
  \PY{n+nf}{msr\PYZus{}s} \PY{n+no}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}\PY{p}{,} \PY{n+no}{x0}
  \PY{n+nf}{mov} \PY{n+no}{x0}\PY{p}{,} \PY{c}{\PYZsh{}0}
  \PY{n+na}{...}

\PY{n+na}{.macro} \PY{n+no}{kernel\PYZus{}exit}\PY{p}{,} \PY{n+no}{el}
  \PY{n+nf}{mrs\PYZus{}s} \PY{n+no}{x20}\PY{p}{,} \PY{n+no}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}
  \PY{n+nf}{mvn} \PY{n+no}{x20}\PY{p}{,} \PY{n+no}{x20}
  \PY{n+nf}{msr\PYZus{}s} \PY{n+no}{SYS\PYZus{}APIBKEYLO\PYZus{}EL1}\PY{p}{,} \PY{n+no}{x20}
  \PY{n+nf}{mov} \PY{n+no}{x20}\PY{p}{,} \PY{c}{\PYZsh{}0}
  \PY{n+na}{...}
\end{Verbatim}


==> code/nonatomic.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c}{\PYZsh{} 1) authentication and use}
\PY{n+nf}{autib} \PY{n+no}{x2}\PY{p}{,} \PY{n+no}{x0}  \PY{c}{\PYZsh{} authenticate}
\PY{n+nf}{blr} \PY{n+no}{x2}        \PY{c}{\PYZsh{} branch or load (use)}

\PY{c}{\PYZsh{} 2) target address calculation and signing}
\PY{n+nf}{adrp} \PY{n+no}{x22}\PY{p}{,} \PY{l+m+mi}{0xffff}\PY{n+no}{..cf000} \PY{c}{\PYZsh{} calculate target address}
\PY{n+nf}{pacib} \PY{n+no}{x22}\PY{p}{,} \PY{n+no}{x23}

\PY{c}{\PYZsh{} 3) re\PYZhy{}signing (authentication and signing)}
\PY{n+nf}{autib} \PY{n+no}{x23}\PY{p}{,} \PY{n+no}{x8}  \PY{c}{\PYZsh{} authenticate}
\PY{n+nf}{pacib} \PY{n+no}{x23}\PY{p}{,} \PY{n+no}{x9}  \PY{c}{\PYZsh{} signing with different context}
\end{Verbatim}


==> code/objbind.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{struct} \PY{n}{irqaction} \PY{p}{\PYZob{}}
  \PY{n}{irq\PYZus{}handler\PYZus{}t} \PY{n}{handler}\PY{p}{;}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
  \PY{k}{const} \PY{k+kt}{char} \PY{o}{*}\PY{n}{name}\PY{p}{;}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{c+cm}{/* This is an annotation given by PAL */}
\PY{p}{\PYZcb{}} \PY{n}{\PYZus{}\PYZus{}attribute\PYZus{}\PYZus{}}\PY{p}{(}\PY{p}{(}\PY{n}{objbind}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{name}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{handler}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{;}
\PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{n}{request\PYZus{}percpu\PYZus{}irq}\PY{p}{(}\PY{k+kt}{unsigned} \PY{k+kt}{int} \PY{n}{irq}\PY{p}{,}
                   \PY{n}{irq\PYZus{}handler\PYZus{}t} \PY{n}{handler}\PY{p}{,}
                   \PY{k}{const} \PY{k+kt}{char} \PY{o}{*}\PY{n}{devname}\PY{p}{,}
                   \PY{k+kt}{void} \PY{n}{\PYZus{}\PYZus{}percpu} \PY{o}{*}\PY{n}{percpu\PYZus{}dev\PYZus{}id}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{n}{irqaction} \PY{o}{*}\PY{n}{action}\PY{p}{;}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
  \PY{n}{action}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{name} \PY{o}{=} \PY{n}{devname}\PY{p}{;}
  \PY{c+cm}{/*}
\PY{c+cm}{   * this will be instrumented like the follows :}
\PY{c+cm}{   * old\PYZus{}ctx = HASH(typeof(handler))}
\PY{c+cm}{   * new\PYZus{}ctx = HASH(typeof(handler)) \PYZca{}}
\PY{c+cm}{               HASH(typeof(*action)) \PYZca{}}
\PY{c+cm}{               (u64)action\PYZhy{}\PYZgt{}name;}
\PY{c+cm}{   * action\PYZhy{}\PYZgt{}handler = CHANGE\PYZus{}CONTEXT(handler,}
\PY{c+cm}{   *                             old\PYZus{}ctx, new\PYZus{}ctx);}
\PY{c+cm}{   */}
  \PY{n}{action}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n}{handler} \PY{o}{=} \PY{n}{handler}\PY{p}{;}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/pac-analogue.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n+na}{.macro} \PY{n+no}{pac\PYZus{}aut\PYZus{}xpac} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{ctx}
  \PY{n+nf}{eor} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{CONSTANT1}
  \PY{n+na}{...}
  \PY{n+nf}{eor} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{ctx}
\PY{n+na}{.endm}

\PY{n+na}{.macro} \PY{n+no}{pacsp\PYZus{}autsp} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{ctx}
  \PY{n+nf}{eor} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{CONSTANT1}
  \PY{n+na}{...}
  \PY{n+nf}{sub} \PY{n+no}{reg}\PY{p}{,} \PY{n+no}{sp}\PY{p}{,} \PY{n+no}{reg}
\PY{n+na}{.endm}
\end{Verbatim}


==> code/pacbind-level3.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+cm}{/* @include/linux/dmaengine.h */}
\PY{k}{struct} \PY{n}{dma\PYZus{}router} \PY{p}{\PYZob{}}
  \PY{k}{struct} \PY{n}{device} \PY{o}{*}\PY{n}{dev}\PY{p}{;}
  \PY{k+kt}{void} \PY{p}{(}\PY{o}{*}\PY{n}{route\PYZus{}free}\PY{p}{)}\PY{p}{(}\PY{k}{struct} \PY{n}{device} \PY{o}{*}\PY{p}{,} \PY{k+kt}{void} \PY{o}{*}\PY{p}{)}\PY{p}{;}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{ifdef CONFIG\PYZus{}KPAC}
\PY{p}{\PYZcb{}} \PY{n}{\PYZus{}\PYZus{}attribute\PYZus{}\PYZus{}}\PY{p}{(}\PY{p}{(}\PY{n}{objbind}\PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{dev}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{route\PYZus{}free}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{;}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{else}
\PY{p}{\PYZcb{}}\PY{p}{;}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{endif}
\end{Verbatim}


==> code/repac-vulnerable.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c}{\PYZsh{} 1) vulnerable re\PYZhy{}signing}
\PY{n+nf}{autib} \PY{n+no}{x22}\PY{p}{,} \PY{n+no}{x8}  \PY{c}{\PYZsh{} x22: an attacker\PYZhy{}chosen pointer}
\PY{n+nf}{pacib} \PY{n+no}{x22}\PY{p}{,} \PY{n+no}{x9}  \PY{c}{\PYZsh{} no exception raises when aut fails}
\PY{n+nf}{str} \PY{n+no}{x22}\PY{p}{,} \PY{p}{[}\PY{n+no}{x10}\PY{p}{]}

\PY{c}{\PYZsh{} 2) secure re\PYZhy{}signing}
\PY{n+nf}{mov} \PY{n+no}{x23}\PY{p}{,} \PY{n+no}{x22}  \PY{c}{\PYZsh{} x22: an attacker\PYZhy{}chosen pointer}
\PY{n+nf}{autib} \PY{n+no}{x23}\PY{p}{,} \PY{n+no}{x8}
\PY{n+nf}{xpaci} \PY{n+no}{x22}
\PY{n+nf}{cmp} \PY{n+no}{x23}\PY{p}{,} \PY{n+no}{x22}
\PY{n+nf}{be} \PY{n+no}{valid}
\PY{n+nf}{ldr} \PY{n+no}{x23}\PY{p}{,} \PY{p}{[}\PY{n+no}{x23}\PY{p}{]} \PY{c}{\PYZsh{} an exception raises when aut fails}
\PY{n+nl}{valid:}
\PY{n+nf}{pacib} \PY{n+no}{x23}\PY{p}{,} \PY{n+no}{x9}
\PY{n+nf}{str} \PY{n+no}{x23}\PY{p}{,} \PY{p}{[}\PY{n+no}{x10}\PY{p}{]}
\end{Verbatim}


==> code/repac.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
  \PY{k}{if} \PY{p}{(}\PY{n}{\PYZus{}\PYZus{}builtin\PYZus{}expect}\PY{p}{(}\PY{n}{target} \PY{o}{!}\PY{o}{=} \PY{l+m+mi}{0}\PY{p}{,} \PY{l+m+mi}{1}\PY{p}{)}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{n}{xpaced} \PY{o}{=} \PY{n}{XPAC}\PY{p}{(}\PY{n}{target}\PY{p}{)}\PY{p}{;}
    \PY{n}{auted} \PY{o}{=} \PY{n}{AUT}\PY{p}{(}\PY{n}{target}\PY{p}{,} \PY{n}{oldContext}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{\PYZus{}\PYZus{}builtin\PYZus{}expect}\PY{p}{(}\PY{n}{xpaced} \PY{o}{=}\PY{o}{=} \PY{n}{auted}\PY{p}{,} \PY{l+m+mi}{1}\PY{p}{)}\PY{p}{)} \PY{p}{\PYZob{}}
      \PY{n}{target} \PY{o}{=} \PY{n}{PAC}\PY{p}{(}\PY{n}{target}\PY{p}{,} \PY{n}{newContext}\PY{p}{)}\PY{p}{;}
    \PY{p}{\PYZcb{}} \PY{k}{else} \PY{p}{\PYZob{}}
      \PY{n}{tmp} \PY{o}{=} \PY{o}{*}\PY{p}{(}\PY{k+kt}{unsigned} \PY{k+kt}{long} \PY{o}{*}\PY{p}{)}\PY{p}{(}\PY{n}{auted}\PY{p}{)}\PY{p}{;}
    \PY{p}{\PYZcb{}}
  \PY{p}{\PYZcb{}}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\end{Verbatim}


==> code/validator-p1.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c}{\PYZsh{} 1) bgmac\PYZus{}chip\PYZus{}reset() from PARTS}
\PY{n+nf}{mov} \PY{n+no}{x19}\PY{p}{,} \PY{n+no}{x0}  \PY{c}{\PYZsh{} x0: first arg of this function}
\PY{n+nf}{mov} \PY{n+no}{w8}\PY{p}{,} \PY{l+m+mi}{0xa3a8}
\PY{n+nf}{ldr} \PY{n+no}{x8}\PY{p}{,} \PY{p}{[}\PY{n+no}{x19}\PY{p}{,} \PY{n+no}{x8}\PY{p}{]}
\PY{n+nf}{blr} \PY{n+no}{x8}       \PY{c}{\PYZsh{} x8: unprotected}

\PY{c}{\PYZsh{} 2) xpac/pac/blr from iPhone\PYZsq{}s CFI}
\PY{n+nf}{ldr} \PY{n+no}{x8}\PY{p}{,} \PY{p}{[}\PY{n+no}{x26}\PY{p}{,} \PY{n+no}{x27}\PY{p}{,} \PY{n+no}{lsl} \PY{l+m+mi}{3}\PY{p}{]}  \PY{c}{\PYZsh{} load from memory}
\PY{n+nf}{xpaci} \PY{n+no}{x8}     \PY{c}{\PYZsh{} cleared}
\PY{n+nf}{paciza} \PY{n+no}{x8}    \PY{c}{\PYZsh{} repacked}
\PY{n+nf}{blraaz} \PY{n+no}{x8}    \PY{c}{\PYZsh{} use}
\end{Verbatim}


==> code/validator-p2.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c}{\PYZsh{} void sort(void *base, ...,}
\PY{c}{\PYZsh{}           int (*cmp\PYZus{}func)(), void (*swap\PYZus{}func)() ...)}
\PY{n+nf}{autib} \PY{n+no}{x2}\PY{p}{,} \PY{n+no}{x0}
\PY{n+nf}{autib} \PY{n+no}{x1}\PY{p}{,} \PY{n+no}{x3}
\PY{n+nf}{stp} \PY{n+no}{x1}\PY{p}{,} \PY{n+no}{x2}\PY{p}{,} \PY{p}{[}\PY{n+no}{x29}\PY{p}{,} \PY{l+m+mi}{144}\PY{p}{]} \PY{c}{\PYZsh{} spilled}
\PY{n+na}{....}
\PY{n+nf}{ldr} \PY{n+no}{x2}\PY{p}{,} \PY{p}{[}\PY{n+no}{x29}\PY{p}{,} \PY{l+m+mi}{144}\PY{p}{]}     \PY{c}{\PYZsh{} reused}
\PY{n+nf}{add} \PY{n+no}{x1}\PY{p}{,} \PY{n+no}{x20}\PY{p}{,} \PY{n+no}{x1}
\PY{n+nf}{mov} \PY{n+no}{x0}\PY{p}{,} \PY{n+no}{x28}
\PY{n+nf}{blr} \PY{n+no}{x2}
\end{Verbatim}


==> code/validator-p3.s.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c}{\PYZsh{} 1) from iPhone\PYZsq{}s CFI}
\PY{n+nf}{mov} \PY{n+no}{x19}\PY{p}{,} \PY{n+no}{x2}         \PY{c}{\PYZsh{} 3rd arg of function}
\PY{n+nf}{ldr} \PY{n+no}{x21}\PY{p}{,} \PY{p}{[}\PY{n+no}{x19}\PY{p}{,} \PY{l+m+mi}{240}\PY{p}{]} \PY{c}{\PYZsh{} load an attacker\PYZhy{}chosen pointer}
\PY{n+nf}{pacia} \PY{n+no}{x21}\PY{p}{,} \PY{n+no}{x8}       \PY{c}{\PYZsh{} sign}
\PY{n+nf}{str} \PY{n+no}{x21}\PY{p}{,} \PY{p}{[}\PY{n+no}{x19}\PY{p}{,} \PY{l+m+mi}{240}\PY{p}{]}

\PY{c}{\PYZsh{} 2) usb\PYZus{}stor\PYZus{}CB\PYZus{}transport() from PARTS}
\PY{n+nf}{adrp} \PY{n+no}{x22}\PY{p}{,} \PY{l+m+mi}{0xffff0000108cf000}  \PY{c}{\PYZsh{} target address calculation}
\PY{n+nf}{add} \PY{n+no}{x22}\PY{p}{,} \PY{n+no}{x22}\PY{p}{,} \PY{l+m+mi}{0x308}
\PY{n+nf}{bl} \PY{l+m+mi}{0xffff0000108cf320}   \PY{c}{\PYZsh{} call usb\PYZus{}stor\PYZus{}msg\PYZus{}common()}
\PY{n+nf}{add} \PY{n+no}{x11}\PY{p}{,} \PY{n+no}{x22}\PY{p}{,} \PY{l+m+mi}{0x0}
\PY{n+nf}{pacia} \PY{n+no}{x11}\PY{p}{,} \PY{n+no}{x23}          \PY{c}{\PYZsh{} sign}
\PY{n+na}{....}
\PY{c}{\PYZsh{}0xffff0000108cf320:    usb\PYZus{}stor\PYZus{}msg\PYZus{}common()}
\PY{n+nf}{stp} \PY{n+no}{x22}\PY{p}{,} \PY{n+no}{x21}\PY{p}{,} \PY{p}{[}\PY{n+no}{sp}\PY{p}{,} \PY{l+m+mi}{48}\PY{p}{]}  \PY{c}{\PYZsh{} spilled}
\PY{n+na}{....}
\PY{n+nf}{ldp} \PY{n+no}{x22}\PY{p}{,} \PY{n+no}{x21}\PY{p}{,} \PY{p}{[}\PY{n+no}{sp}\PY{p}{,} \PY{l+m+mi}{48}\PY{p}{]}  \PY{c}{\PYZsh{} load an attacker\PYZhy{}chosen pointer}
\PY{n+nf}{ret}

\PY{c}{\PYZsh{} 3) from iPhone\PYZsq{}s CFI}
\PY{n+nf}{mov} \PY{n+no}{x19}\PY{p}{,} \PY{n+no}{x0}       \PY{c}{\PYZsh{} 1st arg of function}
\PY{n+na}{....}
\PY{n+nf}{pacia} \PY{n+no}{x19}\PY{p}{,} \PY{n+no}{x20}    \PY{c}{\PYZsh{} sign}
\end{Verbatim}


==> code/xpac-gadget.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{// param6 and param7 are read from memory @0xff0080cc964}
\PY{k+kt}{unsigned} \PY{k+kt}{long} \PY{k+kt}{long} \PY{n+nf}{FUN\PYZus{}fffffff0080ccb88}\PY{p}{(}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
  \PY{k}{do} \PY{p}{\PYZob{}}
    \PY{p}{.}\PY{p}{.}\PY{p}{.}
    \PY{c+c1}{// uVar9 \PYZlt{}\PYZhy{} memory}
    \PY{n}{uVar9} \PY{o}{=} \PY{o}{*}\PY{p}{(}\PY{n}{ulonglong} \PY{o}{*}\PY{p}{)}\PY{p}{(}\PY{n}{lVar12} \PY{o}{+} \PY{n}{uVar7} \PY{o}{*} \PY{l+m+mi}{8}\PY{p}{)}\PY{p}{;}
    \PY{k}{if} \PY{p}{(}\PY{n}{uVar9} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{0}\PY{p}{)} \PY{p}{\PYZob{}}\PY{p}{.}\PY{p}{.}\PY{p}{.}\PY{p}{\PYZcb{}}
    \PY{k}{else} \PY{p}{\PYZob{}}
      \PY{k}{if} \PY{p}{(}\PY{n}{uVar9} \PY{o}{\PYZlt{}} \PY{n}{uParm6} \PY{o}{|}\PY{o}{|} \PY{n}{uParm7} \PY{o}{\PYZhy{}} \PY{l+m+mi}{1} \PY{o}{\PYZlt{}} \PY{n}{uVar9}\PY{p}{)} \PY{k}{break}\PY{p}{;}
      \PY{c+c1}{// uVar9\PYZsq{}s pac is cleared}
      \PY{n}{uVar4} \PY{o}{=} \PY{n}{xpac}\PY{p}{(}\PY{n}{uVar9}\PY{p}{,}\PY{l+m+mi}{0}\PY{p}{)}\PY{p}{;}
      \PY{c+c1}{// re\PYZhy{}paced with zero as context}
      \PY{n}{pcVar5} \PY{o}{=} \PY{p}{(}\PY{n}{code} \PY{o}{*}\PY{p}{)}\PY{n}{paciza}\PY{p}{(}\PY{n}{uVar4}\PY{p}{)}\PY{p}{;}
      \PY{c+c1}{// blraaz: auc with zero and take the branch}
      \PY{n}{pcVar5} \PY{o}{=} \PY{n}{autiaz}\PY{p}{(}\PY{n}{pcVar5}\PY{p}{)}\PY{p}{;}
      \PY{p}{(}\PY{o}{*}\PY{n}{pcVar5}\PY{p}{)}\PY{p}{(}\PY{p}{)}\PY{p}{;}
    \PY{p}{\PYZcb{}}
    \PY{n}{uVar7} \PY{o}{=} \PY{n}{uVar7} \PY{o}{+} \PY{l+m+mi}{1}\PY{p}{;}
  \PY{p}{\PYZcb{}} \PY{k}{while} \PY{p}{(}\PY{n}{uVar7} \PY{o}{\PYZlt{}} \PY{p}{(}\PY{n}{uVar3} \PY{o}{\PYZgt{}}\PY{o}{\PYZgt{}} \PY{l+m+mi}{3} \PY{o}{\PYZam{}} \PY{l+m+mh}{0xffffffff}\PY{p}{)}\PY{p}{)}\PY{p}{;}
  \PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> spec-fig/tbl-ripe.tex <==
\begin{tabular}{c | r | r | r | r}
	\toprule

  \textbf{Config} &
	\textbf{Succeed} &
  \textbf{Probabilistic} &
  \textbf{Failed} &
  \textbf{Not possible} \\

  \midrule

  Default & 114 & 16 & 720 & 2990 \\
  ASan & 8 & 0 & 842 & 2990 \\
  \sys & 8 & 0 & 842 & 2990 \\

  \bottomrule
  
\end{tabular}


==> spec-fig/tbl-server-lighttpd.tex <==
\begin{tabular}{l rrrrrrrrrr}
	\toprule
	\textbf{} 			&
	\bf baseline 						&
	\multicolumn{2}{c}{\bf 2 variants}	&
	\multicolumn{2}{c}{\bf 4 variants}	&
	\multicolumn{2}{c}{\bf 6 variants}	&
	\multicolumn{2}{c}{\bf 8 variants}	&
	\bf Ave.					\\

	\midrule
	Conn. 16 & 20.9 & 22.5 & (7.5\%) & 22.0 & (5.0\%) & 22.4 & (6.9\%) & 21.9 & (4.9\%) & 6.1\% \\ 
	Conn. 64 & 14.7 & 14.9 & (1.3\%) & 14.9 & (1.4\%) & 15.0 & (1.7\%) & 15.3 & (4.1\%) & 2.1\% \\
	Conn. 256 & 10.69 & 11.27 & (5.4\%) & 11.66 & (9.1\%) & 12.0 & (12.1\%) & 12.2 & (14.3\%) & 10.2\% \\
	\midrule
	Ave.	& & & 4.7\% & & 5.2\% & & 7.0\% & & 7.8\% & 6.1\% \\
	
	\bottomrule
\end{tabular}


==> spec-fig/tbl-server-nginx-2.tex <==
\begin{tabular}{l rrrrrrrrrr}
	\toprule
	\textbf{} 			&
	\bf baseline 						&
	\multicolumn{2}{c}{\bf 2 variants}	&
	\multicolumn{2}{c}{\bf 4 variants}	&
	\multicolumn{2}{c}{\bf 6 variants}	&
	\multicolumn{2}{c}{\bf 8 variants}	&
	\bf Ave.					\\

	\midrule
	Conn. 16 & 19.7 & 20.3 & (3.1\%) & 20.1 & (2.2\%) & 20.7 & (5.0\%) & 20.5 & (4.1\%) & 3.6\% \\ 
	Conn. 64 & 15.2 & 15.8 & (3.9\%) & 15.9 & (4.6\%) & 16.2 & (6.4\%) & 16.8 & (10.5\%) & 6.3\% \\
	Conn. 256 & 11.9 & 13.2 & (11.6\%) & 12.9 & (9.0\%) & 13.4 & (12.9\%) & 13.8 & (16.3\%) & 12.3\% \\
	\midrule
	Ave.	& & & 6.2\% & & 5.3\% & & 8.1\% & & 10.3\% & 7.5\% \\
	
	\bottomrule
\end{tabular}


==> spec-fig/tbl-server-nginx-4.tex <==
\begin{tabular}{l rrrrrrrrrr}
	\toprule
	\textbf{} 			&
	\bf baseline 						&
	\multicolumn{2}{c}{\bf 2 variants}	&
	\multicolumn{2}{c}{\bf 4 variants}	&
	\multicolumn{2}{c}{\bf 6 variants}	&
	\multicolumn{2}{c}{\bf 8 variants}	&
	\bf Ave.					\\

	\midrule
	Conn. 16 & 19.0 & 19.0 & (0.1\%) & 19.8 & (3.8\%) & 20.1 & (5.5\%) & 20.0 & (4.9\%) & 3.6\% \\ 
	Conn. 64 & 15.2 & 15.4 & (1.5\%) & 15.5 & (2.2\%) & 16.0 & (5.2\%) & 16.7 & (9.5\%) & 4.6\% \\
	Conn. 256 & 11.2 & 12.4 & (10.8\%) & 12.7 & (13.5\%) & 13.0 & (16.7\%) & 13.4 & (20.1\%) & 15.3\% \\
	\midrule
	Ave.	& & & 4.2\% & & 6.5\% & & 9.1\% & & 11.3\% & 7.8\% \\
	
	\bottomrule
\end{tabular}


==> spec-fig/tbl-server-nginx-8.tex <==
\begin{tabular}{l rrrrrrrrrr}
	\toprule
	\textbf{} 			&
	\bf baseline 						&
	\multicolumn{2}{c}{\bf 2 variants}	&
	\multicolumn{2}{c}{\bf 4 variants}	&
	\multicolumn{2}{c}{\bf 6 variants}	&
	\multicolumn{2}{c}{\bf 8 variants}	&
	\bf Ave.					\\

	\midrule
	Conn. 16 & 18.7 & 18.9 & (1.3\%) & 19.2 & (3.0\%) & 19.9 & (6.5\%) & 20.0 & (7.5\%) & 4.6\% \\ 
	Conn. 64 & 15.2 & 15.4 & (1.3\%) & 15.2 & (0.5\%) & 15.4 & (1.9\%) & 16.4 & (7.9\%) & 2.9\% \\
	Conn. 256 & 11.0 & 11.9 & (7.7\%) & 12.2 & (10.8\%) & 12.8 & (15.7\%) & 13.1 & (19.2\%) & 13.4\% \\
	\midrule
	Ave.	& & & 3.4\% & & 4.8\% & & 8.0\% & & 11.5\% & 6.9\% \\
	
	\bottomrule
\end{tabular}


==> spec-fig/tbl-server-sync.tex <==
\begin{tabular}{c | r | c | rr | rr}
	\toprule

  \textbf{Config} &
	\textbf{Conn} &
  \textbf{Base} &
  \multicolumn{2}{c}{\bf Strict}	& 
  \multicolumn{2}{c}{\bf Selective}	\\

  \midrule

  \cc{lighttpd} & 64    & 10.3  & 11.9  & 15.3\%  & 11.8  & 14.6\% \\
  1 Process   & 512   & 8.71  & 10.5  & 20.5\%  & 10.1  & 15.7\% \\
  1K File     & 1024  & 8.48  & 10.4  & 22.6\%  & 10.1  & 19.3\% \\

  \midrule

  \cc{lighttpd} & 64  & 974   & 994   & 2.05\%  & 992   & 1.85\% \\
  1 Process     & 512 & 959   & 972   & 1.35\%  & 970   & 1.15\% \\
  1M File      & 1024 & 955   & 964   & 0.91\%  & 961   & 0.63\% \\

  \midrule 

  \cc{nginx}    & 64  & 9.81  & 11.6  & 18.7\%  & 11.2  & 14.3\% \\
  4 Threads     & 512 & 8.46  & 10.3  & 21.9\%  & 9.88  & 16.8\% \\
  1K File      & 1024 & 8.20  & 10.2  & 24.4\%  & 9.63  & 17.4\% \\

  \midrule 

  \cc{nginx}    & 64  & 950   & 967   & 1.79\%  & 964   & 1.47\% \\
  4 Threads     & 512 & 985   & 999   & 1.40\%  & 996   & 1.12\% \\
  1M File     & 1024  & 979   & 998   & 1.94\%  & 995   & 1.63\% \\

  \midrule

  Ave. (1KB)    &     &       &       & 20.56\%  &       & 16.4\% \\
  Ave. (1MB)    &     &       &       & 1.57\%  &       & 1.31\% \\
  
  \bottomrule
  
\end{tabular}


==> spec-fig/tbl-taxonomy-mem-error.tex <==
\begin{tabular}{l lll}
\toprule
  \textbf{Memory Error} &\textbf{Main Causes} & \textbf{Defenses}\\
  \midrule
  Out-of-bound r/w		& lack of length check & SoftBound~\cite{softbound} \\
  		 				& format string bug	& ASan~\cite{asan} \\
         & integer overflow & \\
						& bad type casting & \\
  \midrule
  Use-after-free		& dangling pointer & CETS~\cite{cets} \\
  						& double free & ASan~\cite{asan} \\
  \midrule
  Uninitialized read	& lack of initialization & MSan~\cite{msan} \\
						& data structure alignment & \\
						& subword copying & \\
  \midrule
  Undef behavior	& pointer misalignment & UBSan~\cite{ubsan} \\
						& divide-by-zero  & \\
						& null pointer dereference  & \\
\bottomrule                                     
\end{tabular}



==> spec-fig/tbl-vulns.tex <==
\begin{tabular}{c | c | c | c | c}
	\toprule

  \textbf{Program} &
	\textbf{CVE} &
  \textbf{Exploits} &
  \textbf{Sanitizer} &
  \textbf{Detect} \\ 

  \midrule

  nginx-1.4.0 & 2013-2028 & blind ROP & ASan & Yes \\
  cpython-2.7.10 & 2016-5636 & int. overflow & ASan & Yes \\
  php-5.6.6 & 2015-4602 & type confusion & ASan & Yes \\
  openssl-1.0.1a & 2014-0160 & heartbleed & ASan & Yes \\
  httpd-2.4.10 & 2014-3581 & null deref. & UBSan & Yes \\

  \bottomrule
  
\end{tabular}

